Reducing operator complexity in Algebraic Multigrid with Machine Learning Approaches

We propose a data-driven and machine-learning-based approach to compute non-Galerkin coarse-grid operators in algebraic multigrid (AMG) methods, addressing the well-known issue of increasing operator complexity. Guided by the AMG theory on spectrally equivalent coarse-grid operators, we have developed novel ML algorithms that utilize neural networks (NNs) combined with smooth test vectors from multigrid eigenvalue problems. The proposed method demonstrates promise in reducing the complexity of coarse-grid operators while maintaining overall AMG convergence for solving parametric partial differential equation (PDE) problems. Numerical experiments on anisotropic rotated Laplacian and linear elasticity problems are provided to showcase the performance and compare with existing methods for computing non-Galerkin coarse-grid operators.

==> tex/1.1-vcycle.tex <==
\subsection{The V-cycle scheme}

We adopt a somewhat unconventional choice of notations to better inform our algorithmic details later. Let a PDE depend on some parameters $\beta\in\Re^{p}$ and 
\begin{equation}
    \label{eq:param-linear-system}
    \mxA_{\beta}\bfu = \bff
\end{equation}
be its discretized form where $\mxA_{\beta}\in\Re^{N\times N}$ is the discretized differential operator, $\bfu \in \Re^{N}$ is the discretized solution, and $\bff\in\Re^{N}$ is some source term. 
Let $\Omega^l$ denote the space of vectors of dimension $N_l$. On the $l^{th}$ level of the V-cycle scheme, we are given a linear system 
\begin{equation}
\label{eq:lth-level}
\mxA_{g,\beta}^{(l)}\bfe^{(l)} = \bfr^{(l)}
\end{equation}
where $\mxA_{g,\beta}^{(l)}$ is an operator mapping from $\Omega^l$ to $\Omega^l$. Note that \eqref{eq:param-linear-system} is the linear system on the first level and that we assume the $L^{th}$ level is the last level. On the $L^{th}$ level, we simply solve \eqref{eq:lth-level} exactly. Otherwise, a pre-smoothing step is firstly applied by computing 
\begin{equation}
    \label{eq:relaxation}
    \bfe^{(l)} \leftarrow (\mxI-\mxM^{-1} \mxA_{g,\beta}^{(l)}) \bfe^{(l)} + \mxM^{-1} \bfr^{(l)}
\end{equation}
for $\nu$ times to eliminate the error components of high frequencies. $\mxM$ is a pre-determined smoothing operator which we assume to take on the same form consistently throughout the multigrid hierarchy. Let
\[
\mxP^{(l)} : \Omega^{l+1} \rightarrow \Omega^{l}
\]
be the prolongation operator on the $l^{th}$ level and 
\[
\mxR^{(l)} : \Omega^{l} \rightarrow \Omega^{l+1}
\]
denote the restriction operator on the $l^{th}$ level. The system is then projected to the next level by computing
\[
\begin{cases}
\label{eq:galerkin}
\mxA_{g,\beta}^{(l+1)} \leftarrow \mxR^{(l)}\mxA_{g,\beta}^{(l)}\mxP^{(l)}
\\ 
\bfr^{(l+1)}\leftarrow \mxR^{(l)}\left(\bfr^{(l)}-\mxA^{(l)}\bfe^{(l)}\right),\quad \forall \,l \in \{1,2,\ldots, L-1\}.
\end{cases}
\]
A coarse-grid correction step is then applied by doing 
\[
\bfe^{(l)} \leftarrow \mxP^{(l)}\bfe^{(l+1)}
\]
and a post-smoothing step of the same form as \eqref{eq:relaxation} is lastly followed. The algorithmic details are summarized in  \cref{alg:v}.

%% Modify the v-cycle pseudo-code in accordance to the notations above.

\begin{algorithm}
    \caption{The Multigrid V-Cycle Scheme \cite{notay2007convergence}}
    \label{alg:v}
    \begin{algorithmic}[1]
        \REQUIRE $l$, $L$, $\mxA_{\beta}$, $\bff$, $\{\mxP^{(k)}\}_{k=1}^{L-1}$, $\{\mxR^{(k)}\}_{k=1}^{L-1}$, $\mxM$, $\nu$ 
    
        % \hspace{1px}
    
        \ENSURE $\bfu^{(l)}$ such that $\mxA_{\beta}\bfu \approx \bff$ 
    
        % \hspace{1px}
        % \hrule
        % \hspace{1px}

        \STATE Initialize $\bfu^{(l)} = \bfzero$ 
        \STATE Do $\bfu^{(l)} \gets (\mxI-\mxM^{-1} \mxA_{\beta}) \bfu^{(l)} + \mxM^{-1} \bff $ for $\nu$ steps 
        \STATE Compute $\bfr = \bff - \mxA_{\beta}\bfu^{(l)}$
        % \State Let $\mxA_{g,\beta}^{(0)} = \mxA$ and $\bfr_g^{(0)} = \bfr$}
        \STATE Compute $\mxA_{g,\beta}^{(l+1)} = \mxR^{(l)}\mxA_{\beta}\mxP^{(l)}$, $\bfr^{(l+1)} = \mxR^{(l)}\bfr$ 
        \IF{$l+1$ is $L$}
            \STATE Solve for $\bfe^{(l+1)}$ in $\mxA_{g,\beta}^{(l+1)}\bfe^{(l+1)} = \bfr^{(l+1)}$ 
            % \State \Return $\bfe_g^{(l+1)}$
        \ELSE
            \STATE Get $\bfe^{(l+1)}$ by doing V-Cycle with inputs $l+1$, $L$, $\mxA_{g,\beta}^{(l+1)}, \bfr^{(l+1)}$, $\{\mxP^{(k)}\}$, $\{\mxR^{(k)}\}$, $\mxM$, $\nu$ 
        \ENDIF
        \STATE Prolongate and correct: $\bfu^{(l)}\leftarrow\bfu^{(l)}+\mxP^{(l)}\bfe^{(l+1)}$ 
        % \For{$i = 1:\nu$}
        % \State $\bfu \gets (\mxI-\mxM^{-1} \mxA) \bfu + \mxM^{-1} \bff $
        % \EndFor
        \STATE Do $\bfu^{(l)} \gets (\mxI-\mxM^{-1} \mxA_{\beta}) \bfu^{(l)} + \mxM^{-1} \bff $ for $\nu$ steps 
        \RETURN $\bfu^{(l)}$ 
    \end{algorithmic}
\end{algorithm}



==> tex/1.2-related.tex <==
\subsection{Motivation and related works}

When projecting a linear system to the next level, typically the size of the system decreases by a half. One serious issue arising in this process is that although the size gets smaller, the linear operator tends to lose sparsity. This gets more severe as the level goes deeper. To demonstrate this, let us consider the 3-dimensional Poisson's equation 
\begin{equation}
    \label{eq:poisson}
    -\Delta u =f 
\end{equation}
discretized with the seven-point finite difference method on a $100\times 100\times 100$ grid \cite{bienz2016reducing}. The matrix sparsity patterns in the hierarchy of the V-cycle are presented in  \cref{sparsity-pattern}. From the figure, it is clear that the bandwidths of the matrices increase with the level.  \cref{sparsity-table} shows that as the problem size decreases, the average number of nonzeros increases substantially. The diminishing sparsity patterns in coarse grid operators induce a growth in the cost of data communications in parallel solvers. Consequently, a much longer period of time has to be spent for solving the residual equations on coarser-levels.  \cref{communication} shows the total costs partitioned into the local computation cost and the communication cost in multigrid hierarchies for solving \eqref{eq:poisson}. We see from the figure that the decreasing problem size causes a reduction in the cost of the actual computing as the level goes deeper. While this is expected, starting from the first coarse level (level 2), the total computational cost is dominated by the cost of data communications.

\begin{figure}[]
    \centering  \includegraphics[width=0.7\columnwidth]{figs/sparsity.pdf}
    \caption{The sparsity patterns of $\mxA_g^{(1)}$, $\mxA_g^{(4)}$, and $\mxA_g^{(5)}$ in  \cref{alg:v} when using it to solve the 3-dimensional Poisson's equation}
    \label{sparsity-pattern}
\end{figure}  

\begin{table}[H]
    \centering
    \caption[Matrix statistics]{Matrix statistics using classical Multigrid method for 3-D Poisson's equation.}
    \begin{tabular}{c|c|c|c}
       level  & matrix size &non-zero entries & non-zero entries per row\\\hline
        1&1,000,000 & 6,940,000 & 7\\
        2&500,000 &9,320,600 &19 \\
        3&83,338 &2,775,206 &34 \\
        4&10,401 &517,309 & 50\\
        5 & 738 & 30,272 & 42
        % 4&65025 & & \\
    \end{tabular}
    \label{sparsity-table}
\end{table}  

This phenomenon has been observed for quite some time and researchers have attempted to alleviate it with several different approaches. Previous works that take more conventional approaches such as removing weakly connected nodes, minimizing spectral in-equivalence of stencils, and sparsifying smooth aggregations include \cite{falgout2014non, treister2015non, bienz2016reducing}. \textbf{(Add more detailed literature review on existing sparsification approaches.)}

In this work, we take on a different perspective by using deep learning methods, the attention mechanism in particular \cite{vaswani2017attention}, to find sparsified operators on each level. Recently, there has been a line of works exploring the interaction between deep learning and multigrid methods \cite{lecun2015deep}. Two directions in this field have emerged: leveraging the idea behind multigrid to improve deep learning models and improving multigrid methods with deep learning models. 

Works in the former direction include \cite{he2019mgnet} in which the authors attempt to incorporate the multilevel idea to improve convolutional neural networks (CNNs) and \cite{vater2021training} in which a two-level algorithm is proposed for training neural networks. For the latter kind, \cite{luz2020learning, katrutsa2020black, greenfeld2019learning} deal with learning better prolongation (a.k.a. interpolation) operators. \cite{taghibakhshi2021optimization} takes advantage of techniques in deep reinforcement learning to better tackle the problem of optimally partitioning the fine level nodes during coarsening. Both \cite{huang2021learning} and \cite{kuznichov2022learning} focus on the problem of learning better smoothers (relaxation matrices). In the former work, smoothers are directly parameterized by multi-layer CNNs while the latter work focuses on learning to assign better weights to the weighted Jacobi smoothers (see \cite{saad2003iterative} for a detailed discussion on classical smoothers).

% In this work, we consider not only PDEs with fixed parameters but also parametric PDEs in which the parameters are only assumed to be lying in some known distributions. As a result, the original system will become
% \begin{equation}
%     \label{eq:param-linear-system}
%     \mxA_{\beta}\bfu = \bff
% \end{equation}
% and the coarse-level systems at the $l^{th}$ level become
% \begin{equation}
%     \label{eq:param-coarse-system}
%     \mxA_{g,\beta}^{(l)}\bfe^{(l)} = \bfr^{(l)}
% \end{equation}
% where $\mxA_{\beta}$ and $\mxA^{(l)}_{g,\beta}$ depend on $\beta$. Here, $\mxA_{g,\beta}^{(l)}$ denotes the coarse-grid operator in the $l^{th}$ level, $\bfr^{(l)}$ denotes the residual vector projected from the $l-1^{th}$ level, and $\bfe^{(l)}$ denotes the error vector on the $l^{th}$ level. We seek to use deep learning models to extract sparsified spectrally equivalent coarse-grid operators ${\mxA}_{c,\beta}^{(l)}$ for all $l$ and a class of different $\beta$'s. 

\begin{figure}[]
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/communication.png}
    \caption{Communication cost and computation cost in different levels when using multigrid to solve 3-D Poisson's Equation \cite{bienz2020reducing}}
    \label{communication}
\end{figure}

Our contributions are summarized as follows:
\begin{itemize}
    \item We developed an algorithm based on the attention mechanism to sparsify all the coarse-grid operators in the hierarchy of the V-cycle scheme.

    \item \textbf{(What else?)}
\end{itemize}

The rest of the paper is organized as follows. We give a brief review of the attention mechanism and spectral equivalent stencils in  \cref{sec-mg}. We elaborate on our proposed sparsification algorithm in  \cref{sec-spdl}. Numerical experiments and results are presented in  \cref{sec-numerical-exp}. We discuss the limitations of our method and some possible future improvements in  \cref{sec-limitation}. The conclusion comes lastly in  \cref{sec-conclusion}.

==> tex/discarded-tex/2.1-relaxation.tex <==
\subsection{Relaxation Methods}\label{sec:relax}

Again consider a linear system
\begin{equation}
    \label{linear-system}
    \mxA\bfu = \bff
\end{equation}
where $\mxA:=[a_{ij}]\in\Re^{n\times n}$ is a SPD matrix and $\bfu,\bff\in\Re^{n}$ are column vectors. A relaxation method solves for $\bfu$ by taking iterations of the form
\begin{equation}
    \label{relaxation}
    \bfu_{k+1} = (\mxI-\mxM^{-1} \mxA) \bfu_{k} + \mxM^{-1} \bff 
\end{equation}
where $\mxM$ is a so-called relaxation matrix. If we let $\mxG = \mxI-\mxM^{-1} \mxA$, we may rewrite \eqref{relaxation} into 
\begin{equation}
    % \label{relaxation-iteration}
    \bfu_{k+1} = \mxG \bfu_{k} + \mxM^{-1} \bff
\end{equation}
where $\mxG$ is the iteration matrix associated with \eqref{relaxation}.

Suppose $\mxA$ is splitted into three matrices: $\mxA = \mxD - \mxL - \mxU$ where 

\[
\mxD =  \begin{bmatrix}
a_{11} & 0 & \ldots & 0 \\
0 & a_{22} & \ddots & \vdots \\
\vdots & \ddots & \ddots & 0 \\
0 & \ldots & 0 & a_{nn} 
\end{bmatrix},\,
-\mxL =  \begin{bmatrix}
0 & 0 & \ldots & 0 \\
a_{21} & 0 & \ddots & \vdots \\
\vdots & \ddots & \ddots & 0 \\
a_{n1} & \ldots & a_{n,n-1} & 0 
\end{bmatrix},\,
\text{and}\,\,
-\mxU = \begin{bmatrix}
0 & a_{12} & \ldots & a_{1n} \\
0 & 0 & \ddots & \vdots \\
\vdots & \ddots & \ddots & a_{n-1,n} \\
0 & \ldots & 0 & 0 
\end{bmatrix}.
\]

When $\mxM = \mxD$ in \eqref{relaxation}, the method is called the Jacobi method; when $\mxM = w\mxD$ where $0\leq w\leq 1$, it is the weighted Jacobi method; and when $\mxM = \mxD-\mxL$, it becomes the Gauss-Seidel method. 

Let us denote the residual of the $k^{th}$ iterate as $\bfr_k$; that is, 
\begin{equation}
    \label{relaxation-residual}
    \bfr_k:=\bff - \mxA\bfu_k.
\end{equation}
We denote the true solution to \eqref{linear-system} as $\bfu_{*}$; i.e. $\mxA\bfu_* = \bff$. When applying a relaxation method, the approximation error in the ${k+1}^{th}$ iterate is defined as 
\begin{align}
    \notag 
    \bfe_{k+1} &:= \bfu_* - \bfu_{k+1} = \bfe_k - \mxM^{-1}\bfr_k \\
    &= (\mxI - \mxM^{-1}\mxA)\bfe_k = \mxG \bfe_k.
    \label{relaxation-error}
\end{align}
Note that we employed the fact that
\begin{equation}
    \label{residual-eq}
    \bfr_k = \mxA\bfe_k 
\end{equation}
for all $k$ when deriving \eqref{relaxation-error}. Equation \eqref{residual-eq} is called the residual equation; it plays a central role in the formulation of multigrid methods.



==> tex/discarded-tex/2.2-amg.tex <==
\subsection{Algebraic Multigrid}

Multigrid methods can be classified into two categories: geometric multigrid (GMG) and algebraic multigrid (AMG). In GMG, coarsening and interpolating schemes are fixed across the hierarchy. This is done by directly taking the underlying geometric information into account. However, this is typically not available for problems with complicated unstructured meshes. In contrast, in AMG, coarsening and interpolating schemes are adjusted for different levels as per the algebraic properties possessed by the linear systems, making the method widely applicable to a lot of problems. In this work, we focus on the latter case. Also note that we will limit our discussion to the Two-Grid scheme, meaning that we only form a hierarchy of two levels without going deeper. This is because a multigrid scheme can be obtained by simply recursively applying the Two-Grid scheme. For a detailed review of multigrid methods, see \cite{trottenberg2000multigrid, wesseling1995introduction, xu2017algebraic, briggs2000multigrid, stuben2001review, falgout2006introduction}.

As mentioned, relaxation methods form a major component of multigrid methods: they are used to approximate the solution of the linear system on each level. However, while relaxation methods are good at eliminating high-frequency (oscillatory) components in $\bfe_k$, they are known for being notoriously bad at reducing low-frequency (smooth) components. It is worth pointing out that in the context of AMG, smooth (and oscillatory) components are referred as ``algebraically smooth (and oscillatory)" components being distinguished from ``geometrically smooth" components. Geometrically smooth components represent the vectors that are physically smooth if one plots them out. In contrast, algebraically smooth components refer to those which are hard for relaxation methods to eliminate. There are instances where algebraically smooth vectors are geometrically oscillatory \cite{briggs2000multigrid}. 

The main feature of multigrid methods is that they can effectively reduce the smooth components in the error vector $\bfe$ by transferring the original problem to coarse levels. Following \cite{falgout2014non, notay2007convergence}, we consider the symmetric Two-Grid scheme, the algorithmic details of which are summarized in Algorithm \ref{alg:tg}. Choose a relaxation method defined by a relaxation matrix $\mxM$. We first relax the original linear system for $\nu$ iterations to get a rough approximation $\bfu$ to the true solution $\bfu_*$. Define $\bfe_* = \bfu_* - \bfu$. Multiplying both sides by $\mxA$ yields the residual equation on the fine level $\mxA\bfe_* = \bfr$; again $\bfe_*$ is the true solution. We then transfer the residual equation to the coarse level by applying the prolongation operator $\mxP$ and the restriction operator $\mxR$; that is, we compute 
\begin{equation}
\label{eq-coarse-form}
\mxA_g = \mxR\mxA\mxP,\,\,\bfr_g=\mxR\bfr,
\end{equation}
and form the coarse level residual equation $\mxA_g\bfe_g = \bfr_g$. We solve for $\bfe_g$, project it back to the fine level by computing $\bfe = \mxP\bfe_g$ to get a hopefully good approximation to $\bfe_*$, and correct $\bfu$ by $\bfu \leftarrow \bfu + \bfe$. We run $\nu$ iterations of the relaxation method with the relaxation matrix $\mxM^\top$ on the original problem by using the corrected $\bfu$ as the initial guess to get the final approximate solution. Note that the way how $\mxA_g$ is formed in \eqref{eq-coarse-form} is called the Galerkin product. 



==> tex/discarded-tex/2.3-stencil.tex <==
\subsection{Stencil Representations}

We make a quick remark on the stencil representations of matrices. When we use Finite Difference Methods (FDM) or structured Finite Element Methods to discretize PDEs, the resulting stiffness matrix (the matrix that defines the linear system) can be neatly represented by a much smaller matrix, called a stencil. For instance, consider the 2-dimensional Poisson's equation discretized with second-order FDM

\begin{equation}
    \label{4pt-stencil}
    -\Delta u(x_i, y_j) \approx \dfrac{-u_{i+1,j} - u_{i,j+1} + 4u_{i,j} - u_{i-1,j} - u_{i,j-1}}{h^2}
\end{equation}
where $u_{i,j} := u(x_i, y_j) := u(ih,jh)$ and $h$ is the discretization step size.
The stencil representation for \eqref{4pt-stencil} reads 
$
\left[\begin{array}{ccc}
     & -1 & \\
    -1 & 4 & -1 \\
     & -1 &
\end{array}\right].
$
Note that the stencil representation stands for the local interaction (communication) of each node with its neighbors.

==> tex/discarded-tex/2.4-communication.tex <==
\subsection{Increasing Communications}

A serious issue associated with multigrid methods is that although coarse-level matrices have much smaller sizes, they tend to lose sparsity as it gets deeper. 

To demonstrate this issue, let us consider the 3-dimensional Poisson's equation 
\begin{equation}
    \label{eq:poisson}
    -\Delta u =f 
\end{equation}
discretized with the second-order finite difference method on a $100\times 100\times 100$ grid. Figure \ref{sparsity-pattern} shows the matrix sparsity pattern when using classical multigrid to solve \eqref{eq:poisson}. From the figure, it is clear that the bandwidths of the matrices increase as the level gets down. Table \ref{sparsity-table} shows that as the problem size decreases, the average number of nonzeros increases substantially. This decreased sparsity in coarse grid operators causes an increase in the cost for parallel communications. This induces a much longer period of time for solving for the residual equations on coarser-levels than that spent working on the original fine-level
problem. Figure \ref{communication} shows the total costs partitioned into the local computation cost and the communication cost in multigrid hierarchies for solving \eqref{eq:poisson}. We see from the figure that the decreasing problem size makes it cost much less for the actual computing as the method goes deeper. This is expected. However, starting from the first coarse level (level 1), the total computational cost is dominated by the communication cost. 

The reason of why this happens is because when the original system is projected to a coarser level, it introduces more communications between each node and its neighbors. Recall that a stencil representation in fact reflects the local interaction. Since coarsening induces more interactions, the corresponding stencil representation of the coarse-level matrix tends to get denser. Therefore, the matrix on the coarser level then will have more non-zero entries. As the dimension of the problem gets higher, the problem will get much worse.



==> tex/discarded-tex/3.4-implementation.tex <==
% do we want to discuss some implementation details as well? 
